Quantum Positional Encodings for Graph Neural Networks

In this work, we propose novel families of positional encodings tailored to graph neural networks obtained with quantum computers. These encodings leverage the long-range correlations inherent in quantum systems that arise from mapping the topology of a graph onto interactions between qubits in a quantum computer. Our inspiration stems from the recent advancements in quantum processing units, which offer computational capabilities beyond the reach of classical hardware. We prove that some of these quantum features are theoretically more expressive for certain graphs than the commonly used relative random walk probabilities. Empirically, we show that the performance of state-of-the-art models can be improved on standard benchmarks and large-scale datasets by computing tractable versions of quantum features. Our findings highlight the potential of leveraging quantum computing capabilities to enhance the performance of transformers in handling graph data.

==> proof_sachin.tex <==

\section{Theoretical part of the paper}
In this section we present proofs relating the expressiveness of QW with well known WL tests and other graph invariants like the Furer Invariant \cite{Furer2010}.  

\subsection{Proof of proposition \ref{pr:1QW-uni}}
 $1$-QW $\sqsubset$ $1$-WL when the input state of the unitary is a uniform superposition state.
 \newline We show that beginning with an initial uniform superposition state, the action of ${\mathcal{H_{XY}}}$ evolution is similar to WL coloring iterations. We consider a graph $\mathcal{G}$, with vertex set $\mathcal{V}$ and consisting of $N$ nodes. Suppose we begin with 1 particle QW. The action of ${\mathcal{H_{XY}}}$ restricted to 1-particle subspace is then equivalent to action of the adjacency matrix $A$. 
Therefore we have :
\begin{equation}
\begin{split}
    e^{\ii\mathcal{H_{XY}}t}& = \Sum_{k = 0} ^{\infty} \frac{(\ii.t)^k}{k!} (H_{XY})^k \\
    & \equiv 1 + \ii At + \ii^2\frac{1}{2}A^2t^2+..
\end{split}
\end{equation}

The action of $A$ on the identity vector is simply the vector of degrees of the nodes, which is the first WL iteration. Further operating with $A$ leads to a vector where we add degrees of the neighbours of a node. Further iterations simply lead to vectors where two entries are equal if they have same degrees and equal number of neighbours also of same degrees, which corresponds to stable WL coloring. This scheme corresponds exactly to a $1$-WL test with the sum operation as the update function.
To see this, suppose we define $|I\rangle$ as the normalized vector of uniform superposition. Each entry of the vector is $\frac{1}{\sqrt{N}}$. After the action of adjacency matrix $A$ we obtain the vector $|I^{(1)}\rangle$, which will be:
\begin{equation}
	|I^{(1)}\rangle = \frac{1}{\sqrt{N}}\begin{bmatrix}
				d_1\\
				d_2\\
				..\\
				..\\
				d_N
			\end{bmatrix}
\end{equation}  
where $d_1,d_2,...,d_N$ are the degrees of the nodes. This can be interpreted as the first step of WL coloring where each node is assigned the color depending on the degree. Again applying $A$ to vector $|I^{(1)}\rangle$ we obtain the vector $|I^{(2)}\rangle$, which will be:
\begin{equation}
	|I^{(1)}\rangle = \frac{1}{\sqrt{N}}\begin{bmatrix}
				\sum_{i\in \mathcal{N}(1)}d_i\\
				\sum_{i\in \mathcal{N}(2)}d_i\\
				..\\
				..\\
				\sum_{i\in \mathcal{N}((N)}d_i
			\end{bmatrix}
\end{equation}  
where $\mathcal{N}(i)$ is the set of neighbours of node $i$. Thus in this iteration, the degrees of the neighbours of a node are aggregated \footnote{Again, we are here in a case where the aggregation function is the sum operation, which is not an injective function. This is the main reason for which the $1-QW$ is less powerful than the $1-WL$, which allows any sort of aggregation functions and most notably injective functions.}. Further steps simply lead to aggregation of neighbour properties for a given node until stable coloring is reached i.e same colored neighbours will have same entry in the vector.
It is known that $i^{th}$ entry of $A^{k}|\boldsymbol{1}\rangle$ will correspond to the number of walks of length $k$ beginning from node $i$. Every $k^{th}$ iteration induces a refinement on the previous step until convergence. It has been shown that stable WL coloring is a refinement of the partition obtained at convergence for some $k$ for $A^{k}|\boldsymbol{1}\rangle$ and is in fact equal for a large number of graphs \cite{Powers1982}.  Since the evolution due to $\mathcal{H_{XY}}$ is simply the weighted summation of these vectors, it follows that that the output vector for 1-QW with input superposition $\sqsubset$ 1-WL.



\subsection{Proof of proposition \ref{th:1QW-loc}}

$2$-WL $\sqsubseteq$ $1$-QW $\sqsubseteq$ $1$-WL  when the input state of the unitary is a localized state.
\newline The complete proof relies on this two following statements :
\begin{enumerate}
    \item 1-WL $\leq$ 1-QW when the input state of the unitary is a localized state. \newline 
    We can see that in fact for a general input state a single-particle QW can be more expressive than a 1-WL test. For example, beginning with a particle localized at one of the nodes, the action of the ${\mathcal{H_{XY}}}$ as seen above has contributions from different powers of $A$. Beginning with a localized input state, the $k^{th}$ power of $A$ tell about the number of paths of length $k$ between a set of nodes. If 2 regular graphs differ in these quantities, the set of probabilities $p_{ij}=p(i\rightarrow j)$ or probability of a particle to go from node $i$ to $j$ will be different. Thus, a single particle QW can distinguish 2 such regular graphs. However, we know that a 1-WL cannot distinguish regular graphs. Hence 1-QW $\ge$ 1-WL. 

    \item 1-QW $\leq$ F.I when the input state of the unitary is a localized state. \newline
    For a general input and output state, the time averaged transition probability for evolution with $\mathcal{H_{XY}}$ to go from $|\psi\rangle$ to $|\phi\rangle$ is given by:

\begin{equation}
p(|\phi\rangle \rightarrow |\psi\rangle) = lim_{T  \rightarrow \infty}\int_{0}^{T} dt |\langle \phi |e^{i\mathcal{H_{XY}}t}|\psi\rangle|^2 dt
\end{equation}
This can be further written as

\begin{equation}\label{qw_probs}
   p_{|\psi\rangle \rightarrow |\phi\rangle}(\infty) = \sum_{\lambda \in Sp({\mathcal{H_{XY}}})} |\langle \phi |P^\lambda |\psi\rangle |^2 
\end{equation}
where ${\mathcal{H_{XY}}}= \sum_{\lambda \in Sp({\mathcal{H_{XY}}})} \lambda P^{\lambda}$, $Sp({\mathcal{H_{XY}}})$ is the set of eigenvalues of $\mathcal{H_{XY}}$. For a single particle QW, this set is exactly the set of eigenvalues of $A$. $P^\lambda$ are the projectors into the eigenspace spanned by the corresponding eigenvectors. \cite{Furer2010} defines the spectral invariant based on projectors $P^{\lambda}$. We refer to this as the Furer Invariant (F.I.). 
The Furer invariant is a spectral invariant defined in terms of projectors $P^\lambda$ defined above. The projector $P^\lambda$ by definition can be written as $|e_\lambda\rangle \langle e_\lambda|$, where $|e_{\lambda}\rangle$ is the eigenvector corresponding to the eigenvalue $\lambda$. In matrix form this can be written as 
\begin{equation}
	P^\lambda = \begin{bmatrix}
			p^{\lambda}_{11}&p^{\lambda}_{11}&..&p^{\lambda}_{1n}\\
			p^{\lambda}_{21}&p^{\lambda}_{22}&..&p^{\lambda}_{2n}\\
			.&.&.\\
			.&.&.\\
			p^{\lambda}_{n1}&p^{\lambda}_{n2}&..&p^{\lambda}_{nn}\\
   \end{bmatrix}
\end{equation}
The quantities $\langle b_i|P^\lambda|b_j\rangle$ and $\langle b_i|P^\lambda|b_i\rangle$ represent the non-diagonal and the diagonal entries of the matrix $P^{\lambda}$ respectively. The $|b_i\rangle$ represent the coordinate basis vectors where a vector $|0_1,0_2..,1_i,0..,0\rangle $ would represent the node $i$. The quantity $\langle b_i|P^\lambda|b_j\rangle$ represents the product of angles made by the coordinate basis vectors corresponding to node $i,j$ with the eigenspace defined by $\lambda$. Similarly $\langle b_i|P^\lambda|b_i\rangle$ represents the angle made by the coordinate basis vector of node $i$ with the eigenspace defined by $\lambda$. These quantities along with the spectra of the adjacency matrix define the Furer invariant. Expanding each of the vectors $|\phi\rangle$ and $|\psi\rangle$ in terms of the eigenvectors, it can be seen that the probability $p(i \rightarrow j)$ can be computed using the Furer invariant. Thus, the set of probabilities is weaker than the Furer invariant. 


Based on equation \ref{qw_probs}, we see that 1-QW$<$F.I. Therefore, 1-QW$\ge$ 1-WL and 1-QW$<$F.I. In \cite{Rattan2023}, the authors prove that F.I$<$2-WL. Therefore 1-QW$\ge$ 1-WL with input localized state and 1-QW$<$ 2-WL. These inequalities along with Proposition 1.1 tell us that 1-QW $\not\sqsubseteq$ 1-WL and 1-QW $\sqsubseteq$ 2-WL.
    
\end{enumerate}
\subsection{Proof of proposition \ref{pr:kQW}}

$k$-QW $\sqsubset$ to  $k$-$\delta$-LWL for uniform input superposition.
\newline 
For a general $k$-particle case, the WL coloring for a $k$-particle occupation graph is the same as $k$-$\delta$-LWL coloring as defined in \cite{Morris2020}. This is because the colors of the $k$-tuples are updated only based on the local neighbourhood, as is the case for the $k$-$\delta$-LWL test. The k-particle occupancy graph $G^{k}$ is constructed in the following way.: We begin with a $k$-tuple , $(v_1,v_2,..v_{i},v_{i+1},..v_k)$. An adjacent $k$-tuple is found by  replacing $v_i$ with a node $w_i$ such that $w_{i}\in\mathcal{N}(v_i)$. In a $k$-$\delta$-LWL test, colors of a particular $k$-tuple are updated based on colors of the $\it{local}$ neighborhood, in which two $k$-tuples $(v_1,v_2,..v_{i},v_{i+1},..v_k)$ and $(v_1,v_2,..w_{i},v_{i+1},..v_k)$ are local neighbours only if $w_{i}\in\mathcal{N}(v_i)$ in the original graph. Thus the updates for both the cases are equivalent. Analogously to the $1$-QW case, we see therefore that $k$-QW $\sqsubset$ to  $k$-$\delta$-LWL.

\subsection{Proof of proposition \ref{pr:GD-RRWP_SRG}}
One can show \citep{shiau2003physically, gamble2010two} that for strongly regular graphs, the powers of the adjacency matrix $A$ can be expressed as $$A^n = \alpha_n I + \beta_n J + \gamma_n A$$ where $\alpha_n$, $\beta_n$, $\gamma_n$ only depend on $N, k, \lambda, \mu$. $I$ is the identity matrix, $J$ is the matrix full of 1s.\newline The degree matrix is also equal to $kI$, then $(D^{-1}A)^n = A^n/k^n$. Hence the information about distance contained in $\mathbf{P}_{uv}$ for strongly regular graphs is the same as in their adjacency matrices. Therefore, for strongly regular graphs, the GD-WL with RRWP test is equivalent to the WL test.
The F.I. consists of eigenvalues and eigenvectors. It has been shown that F.I $>$ $1$-WL, but weaker than $2$-WL \cite{Rattan2023}. Therefore, $GD$-WL along with eigenvectors cannot distinguish SRGs, which require $3$-WL or higher. 


\subsection{proof of proposition \ref{pr:GD-Ising}}
In this proof, we provide the full calculation for 

\begin{itemize}
    \item The average value of the global occupation observable $\langle \hat n (t) \rangle_\Graph = \langle \Sum_{v \in \mathcal{V}} \hat n_v(t)\rangle_\Graph $
    \item the correlation matrix for the local occupation observables $C_{uv}(t) = \langle \hat n_{u}(t) . \hat n_{v}(t) \rangle_\Graph -  \langle \hat n_{u}(t)\rangle_\Graph  \langle \hat n_{v}(t) \rangle_\Graph$
\end{itemize}
We provide for each of these cases a formulation involving the corresponding graph quantities. In each of these steps, the goal is to show that it is not a powerful tool to distinguish graphs, and more specifically, that it fails to distinguish non isomorphic strongly regular graphs from the same family. 

We start by defining the following quantities : 

\begin{equation}\hat n_{v} = \frac{1}{2}(\mathbb{I} - \hat Z_v)
\end{equation} 
and
\begin{equation}
 \hat Z_v = \displaystyle\bigotimes_{u<v}\mathbb{I}\otimes\hat Z\otimes\displaystyle\bigotimes_{u>v}\mathbb{I}
 \end{equation} 
We also define 
\begin{equation}
    \langle \hat{\mathcal{O}} \rangle_\Graph = \langle \psi_\Graph | \hat{\mathcal{O}} | \psi_\Graph \rangle
    \label{eq:val_moy}
 \end{equation} 
where 
\begin{equation}
   |\psi_\Graph \rangle = \mathcal{U}_\Graph |\psi_0 \rangle  = \mathcal{U}_\Graph \bigotimes_{v =1}^{n}|0 \rangle 
 \end{equation} 
For our case, the evolution operator $ \mathcal{U}_\Graph $ can be written as : 
\begin{equation}
\mathcal{U}_\Graph(\vartheta, t) = \e^{i \Ham_M \vartheta}\e^{-i \Ham_I t} \e^{-i \Ham_M \vartheta}
\end{equation}
where, for a graph $\Graph = (\mathcal{V},\edges)$ we have  
\begin{equation}
    \Ham_{I} = \Sum_{(v,u)\in\edges} \hat n_v \hat n_u + \Sum_{v \in \vertices} \hat n_v 
\end{equation}
		 
 and \footnote{Physically, this describes the same phenomenon as if we had chosen a mixing hamiltonian with operators $X_i$, up to a gauge change. Which leads to similar results that do not affect the statement in the corresponding proposition.}
 \begin{equation}
     \Ham_M=  \Sum_{v\in\mathcal{V}} \hat Y_v
 \end{equation}
 
This corresponds to a single layer Ising evolution, preceded and followed by an evolution through the mixing hamiltonian $\Ham_M$ with opposite signs. The motivation for switching signs in the mixing hamiltonian parameter $\vartheta$ is to allow us to write  $\mathcal{U}_\Graph(\vartheta, t) = \mathcal{U}^{\dag}_M(\vartheta)\cdot\mathcal{U}_I(t) \cdot \mathcal{U}_M(\vartheta)$ which is equal to the identity when $t = 0$. 
\newline Now let us compute the quantities $ \langle \hat n_{v} \hat n_{u}  \rangle_\Graph$ and $\langle \hat n_{v} \rangle_\Graph$

We start by defining the following pulse operator, that will be useful later in this calculation :
\begin{equation}
    \hat{P}^\dagger_\vartheta = \exp\left(-\ii\,\vartheta \Sum_v \hat Y_v\right)=\Prod_v\underbrace{\left[\Cos\,\Id+\Sin\left(\hat\sigma_v^+-\sigma_v^-\right) \right]}_{\hat{P}^\dagger_{\vartheta,v}}
\end{equation}		

where we introduce the spin operators $\hat\sigma^+$ and $\hat\sigma^-$, such that
			
			\begin{equation}
				\begin{array}{cc}
					\hat\sigma^+|0\rangle = |1\rangle,	&	\hat\sigma^+|1\rangle = 0,\\
					\hat\sigma^-|0\rangle = 0,			&	\hat\sigma^-|1\rangle = |0\rangle,
				\end{array}
			\end{equation}
   such that
		       $\hat X = (\hat\sigma^++\hat\sigma^-)/2,\hat Y =-\ii(\hat\sigma^+-\hat\sigma^-)/2$ and
			$\hat Z =\hat\sigma^+\hat\sigma^-$.
\subsubsection{State preparation}
    \begin{enumerate}
        \item We start with the system in 
            \begin{equation}
                |{\bf 0}\rangle = \displaystyle \bigotimes_v |0\rangle.
            \end{equation}
        \item We then apply a pulse of angle $\vartheta$ to get the system in the state
            \begin{equation}
                |\psi_{\vartheta}(0)\rangle = \hat{P}^\dagger_\vartheta|{\bf 0}\rangle=(\Cos)^N\Sum_{\sigma\in\{0,1\}^N} (\Tan)^{n_\sigma}|\sigma\rangle.
            \end{equation}
        \item We then let the system evolve with the Ising Hamiltonian, so that
            \begin{equation}
                |\psi_{\vartheta}(t)\rangle = \e^{-\ii \Ham_I t}|\psi_{\vartheta}(0)\rangle=(\Cos)^N\Sum_{\sigma\in\{0,1\}^N} (\Tan)^{n_\sigma}\e^{-\ii E^{(I)}_\sigma}|\sigma\rangle.
            \end{equation}
        \item Finally, the inverse pulse is then applied, to get
            \begin{equation}
                |\psi_{f,\vartheta}(t)\rangle = \hat{P}_\vartheta|\psi_{\vartheta}(t)\rangle =(\Cos)^N\Sum_{\sigma\in\{0,1\}^N} (\Tan)^{n_\sigma}\e^{-\ii E^{(I)}_\sigma t}\left(\Prod_{v=1}^N\hat{P}_{\vartheta,v}\right)|\sigma\rangle.
            \label{eq:ref_eq}
            \end{equation}
    \end{enumerate}

\subsubsection{Computation of the total occupation}
We first start by providing a full expression, in terms of graph quantities, for a (graph level) observable that we call the global occupation : 
\begin{equation}
    \hat{n}= \Sum_v\hat{n}_v =\Sum_v \hat\sigma^+_v\hat\sigma^-_v,
\end{equation}

Such that, when transposed in the expression provided in equations \ref{eq:ref_eq} and \ref{eq:val_moy} we have : 

\begin{equation}
     \langle \hat n(t) \rangle = (\Cos)^{2N}\Sum_{\sigma,\sigma'\in\{0,1\}^N} \e^{-\ii \left(E^{(I)}_\sigma-E^{(I)}_{\sigma'}\right)t}
                    \underbrace{(\Tan)^{n_\sigma+n_{\sigma'}}
                    \langle\sigma'|\left(\Prod_{v'=1}^N\hat{P}^\dagger_{\vartheta,v'}\right)\hat n \left(\Prod_{v=1}^N\hat{P}_{\vartheta,v}\right)|\sigma\rangle}
                    _{:=f_{\sigma\sigma'}(\vartheta)}.
\end{equation}

We then insert an identity $\Id = \Sum_{\mu \in \{0,1\}^N} |\mu\rangle\langle\mu|$, so that
\begin{equation}
    \label{eq:noft_lambda}
    \langle \hat n(t) \rangle= (\Cos)^{2N}\Sum_{\sigma,\sigma'\in\{0,1\}^N} \e^{-\ii \left(E^{(I)}_\sigma-E^{(I)}_{\sigma'}\right)t}(\Tan)^{n_\sigma+n_{\sigma'}}\Sum_{\mu \in \{0,1\}^N} 
                    n_\mu 
                    \underbrace{\langle\sigma'|\left(\Prod_{v'=1}^N\hat{P}^\dagger_{\vartheta,v'}\right)|\mu\rangle
                    \langle\mu|\left(\Prod_{v=1}^N\hat{P}_{\vartheta,v}\right)|\sigma\rangle}_{=
                    \Prod_{v=1}^N
                    \langle\sigma'_v|\hat{P}^\dagger_{\vartheta,v}|\mu_v\rangle
                    \langle\mu_v|\hat{P}_{\vartheta,v}|\sigma_v\rangle}.
\end{equation}

Let us now compute an expression for the matrix elements appearing in \eqref{eq:noft_lambda} :
\begin{equation}
    \begin{array}{lcl}
    \lambda_{\mu_v\sigma_v}(\vartheta) &:=& \langle\mu_v|\hat{P}_{\vartheta,v}|\sigma_v\rangle \\
                                &=& \Cos\, \langle\mu_v|\sigma_v\rangle +  \Sin\, \langle\mu_v|\hat\sigma^-_v|\sigma_v\rangle -  \Sin\, \langle\mu_v|\hat\sigma_v^+|\sigma_v\rangle\\
                                &=& \Cos\, \delta_{\mu_v,\sigma_v} +  \Sin\, \left(\delta_{\mu_v,\sigma_v-1} -  \delta_{\mu_v,\sigma_v+1}\right)
    \end{array}
\end{equation}

%					The following table gives the possible values for the product $\lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta)$ :
%				        	\begin{equation}
%				        		\label{eq:table}
%				        		\begin{array}{|c|c|}\hline
%				        			(\mu_v,\sigma_v,\sigma'_v)	&	\lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta)\\\hline\hline
%				        			(0,0,0)					&	\Cos^2\\
%				        			(0,1,0)					&	\Cos\Sin\\
%				        			(0,0,1)					&	\Cos\Sin\\
%				        			(0,1,1)					&	\Sin^2\\
%				        			(1,0,0)					&	\Sin^2\\
%				        			(1,1,0)					&	-\Cos\Sin\\
%				        			(1,0,1)					&	-\Cos\Sin\\
%				        			(1,1,1)					&	\Cos^2\\\hline
%				        		\end{array}
%				        	\end{equation}
%					
The following table gives the possible values for the product $\lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta)$ :
        \begin{equation}
            \label{eq:table}
            \begin{array}{|c|c|}\hline
                (\mu_v,\sigma_v,\sigma'_v)	&	\lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta)\\\hline\hline
                (0,0,0),(1,1,1)				&	\Cos^2\\
                (0,1,1),(1,0,0)				&	\Sin^2\\
                (0,1,0),(0,0,1)				&	\Cos\Sin\\
                (1,1,0),(1,0,1)				&	-\Cos\Sin\\\hline
            \end{array}
        \end{equation}

In order to further explicit \eqref{eq:noft_lambda}, we split the set of all vertices into $\mathcal{O}_{\sigma\sigma'} = \{ v | \sigma_v = \sigma'_v=1\}$, $\mathcal{Z}_{\sigma\sigma'} = \{ v | \sigma_v = \sigma'_v=0\}$ and 
$\Delta_{\sigma\sigma'} = \{ v | \sigma_v \neq \sigma'_v\}$, respectively containing $n_0, n_1$, and $n_{\neq}$ vertices, so that 
\begin{equation}
        \Prod_{v=1}^N\lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta) =
    \Prod_{v\in\mathcal{O}_{\sigma\sigma'}}\underbrace{\lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta)}_{=(\Cos)^{2{\mu_v}}(\Sin)^{2-2{\mu_v}}}
    \Prod_{v\in\mathcal{Z}_{\sigma\sigma'}}\underbrace{\lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta)}_{=(\Cos)^{2-2{\mu_v}}(\Sin)^{2{\mu_v}}}
    \Prod_{v\in\Delta_{\sigma\sigma'}}\underbrace{\lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta)}_{\Cos\Sin(-1)^{{\mu_v}}}.
\end{equation}	

We then split $\mu$ in $\mu = \mu^{(1)} \cup \mu^{(0)} \cup \mu^{(\neq)}$, where $\mu^{(1)}=\{\mu_v|v\in\mathcal{O}_{\sigma\sigma'}\}$, $\mu^{(0)}=\{\mu_v|v\in\mathcal{Z}_{\sigma\sigma'}\}$
and $\mu^{(\neq)}=\{\mu_v|v\in\Delta_{\sigma\sigma'}\}$. We can then write
\begin{equation*}
        f^\mu_{\sigma\sigma'}(\vartheta)=\Prod_{v=1}^N\lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta) =\underbrace{
    (\Sin)^{2n_1}(\Tan)^{-2n_{\mu^{(1)}}}\times
    (\Cos)^{2n_0}(\Tan)^{2n_{\mu^{(0)}}}\times
    (\Cos)^{n_{\neq}}(\Sin)^{n_{\neq}}(-1)^{n_{\mu^{(\neq)}}}}
    _{ (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}(\Tan)^{2(n_{\mu^{(0)}}-n_{\mu^{(1)}})} (-1)^{n_{\mu^{(\neq)}}} }.
\end{equation*}	
Noting that $\Sum_{\mu\in\{0,1\}^m} A(n_{\mu}) = \Sum_{p=0}^m\binom{m}{p}A(p)$ we can write
\begin{equation*}
%						\Sum_{\mu \in \{0,1\}^N} n_\mu \Prod_{v=1}^N \lambda^*_{\mu_v\sigma'_v}(\vartheta)\lambda_{\mu_v\sigma_v}(\vartheta) = (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_0}
    \Sum_{\mu \in \{0,1\}^N} n_\mu f^\mu_{\sigma\sigma'}(\vartheta) = \underbrace{(\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}
    \underbrace{
    \Sum_{p_1=0}^{n_1}\binom{n_1}{p_1}
    \underbrace{
    \Sum_{p_0=0}^{n_0}\binom{n_0}{p_0}(\Tan)^{2(p_0-p_1)}
    \underbrace{\Sum_{p_{\neq}=0}^{n_{\neq}}\binom{n_{\neq}}{p_{\neq}}
    \left(p_1+p_0+p_{\neq}\right)
     (-1)^{p_{\neq}}}_{=(p_1+p_0)\delta_{0,n_{\neq}} - \delta_{1,n_{\neq}} }}
     _{=\left[1+(\Tan)^{2}\right]^{n_0}\left[\delta_{0,n_{\neq}}\left(p_1+n_0\frac{(\Tan)^{2}}{1+(\Tan)^{2}}\right)  - \delta_{1,n_{\neq}}\right]      }
     }
     _{=\left[1+(\Tan)^{2}\right]^{n_0}\left[1+(\Tan)^{-2}\right]^{n_1}\left\{\delta_{0,n_{\neq}}\left[n_0(\Sin)^2+n_1\frac{(\Tan)^{-2}}{1+(\Tan)^{-2}}\right]-\delta_{1,n_{\neq}}\right\}}}_
     {
     (\Cos)^{2N}(\Tan)^{n_{\neq}}\left[1+(\Tan)^{2}\right]^{n_0+n_1}\left\{\delta_{0,n_{\neq}}\left[n_0(\Sin)^2+n_1(\Cos)^2\right]-\delta_{1,n_{\neq}}\right\}
     }
\end{equation*}

Since $n_0+n_1+n_{\neq}=N$, 
\begin{equation}
    \label{eq:intermediate1}
     (\Cos)^{2N}(\Tan)^{n_{\neq}}\left[1+(\Tan)^{2}\right]^{n_0+n_1} = \frac{(\Tan)^{n_{\neq}}}{\left[1+(\Tan)^{2}\right]^{n_{\neq}} }=(\Cos\Sin)^{n_{\neq}},
\end{equation}

so that
    
\begin{equation}
    \Sum_{\mu \in \{0,1\}^N} n_\mu f^\mu_{\sigma\sigma'}(\vartheta) =
        \delta_{0,n_{\neq}}\left[n_0(\Sin)^2+n_1(\Cos)^2\right]-\delta_{1,n_{\neq}}\Cos\Sin
\end{equation}




The sum in \eqref{eq:noft_lambda} then only runs on pairs of configuration $(\sigma,\sigma')$ that differ by at most 1 element. Let us simplify those terms.

\begin{itemize}
    \item {\bf $n_{\neq} = 0$} \\
        Then $\sigma=\sigma'$, so that $n_\sigma=n_{\sigma'}=n_1=N-n_0$. 
%							The previous expression then becomes \\
%							$(\Cos)^{2N}(\Tan)^{n_{\neq}}\left[1+(\Tan)^{2}\right]^{n_0+n_1}=(\Cos)^{2N}\left[1+(\Tan)^{2}\right]^N=1$, and
%								\begin{equation}
%									 (\Cos)^{2N}(\Tan)^{2n_\sigma}\Sum_{\mu\in\{0,1\}^N}n_\mu f^\mu_{\sigma\sigma'}(\vartheta)
%									=(\Cos)^{2N}(\Tan)^{2n_\sigma} \left[(N\sin^2\vartheta+n_\sigma(\cos^2\vartheta-\sin^2\vartheta)\right]
%%									=(\Cos)^{2N}(\Sin)^{2n_\sigma} \left[(N-2n_\sigma)(\Cos)^2 +n_\sigma\right]
%								\end{equation}
        \begin{equation}
            f_{\sigma\sigma}(\vartheta) =(\Tan)^{2n_\sigma}\left[(N-n_\sigma)(\Sin)^2+n_\sigma(\Cos)^2\right]
        \end{equation}
    \item {\bf $n_{\neq} = 1$} 
        \begin{itemize}
            \item{$n_{\sigma'} = n_\sigma+1 $ } \\
                Then $n_1=n_\sigma=N-n_0-1$, so that
            \begin{equation}
                \label{eq:sigleqsigp}
                f_{\sigma\sigma'}(\vartheta) = -(\Tan)^{2n_\sigma+1}\Cos\Sin = -(\Tan)^{2n_\sigma}\sin^2\vartheta
            \end{equation}									
            \item{$n_{\sigma'} = n_\sigma-1 $ } \\
                Then $n_1=n_{\sigma'}=N-n_0-1$, so that
            \begin{equation}
                \label{eq:siggeqsigp}
                f_{\sigma\sigma'}(\vartheta) = -(\Tan)^{2n_\sigma-1}\Cos\Sin = -(\Tan)^{2n_\sigma}\cos^2\vartheta
            \end{equation}
        \end{itemize}
        
        {\bf Remark :} Exchanging $\sigma$ and $\sigma'$ in either of the previous equations \eqref{eq:sigleqsigp} or \eqref{eq:siggeqsigp} yields the other one,
        ensuring that $\langle \hat n(t) \rangle$ is real. For example, if $n_{\sigma'} = n_\sigma+1 $
        \begin{equation}
            f_{\sigma'\sigma}= -(\Tan)^{2n_\sigma'}\cos^2\vartheta = -(\Tan)^{2n_\sigma+2}\cos^2\vartheta =  -(\Tan)^{2n_\sigma}\sin^2\vartheta = f_{\sigma\sigma'}
        \end{equation}
\end{itemize}



					
						For a given configuration $\sigma$, we note $\Delta_{\sigma,v}=E_\sigma-E_{\sigma'(v)}$ where $\sigma'(v)$ is the configuration obtain from $\sigma$ by flipping
						$\sigma_v$. The total occupation is then
						
						\begin{equation}
							\langle \hat n(t) \rangle = \Sum_{\sigma\in\{0,1\}^N}\left\{
							f_{\sigma\sigma}(\vartheta)+
							\Sum_{v\in\mathcal{Z}_\sigma}\e^{-\ii\Delta_{\sigma,v}t}f_{\sigma\sigma'(v)}(\vartheta)+
							\Sum_{v\in\mathcal{O}_\sigma}\e^{-\ii\Delta_{\sigma,v}t}f_{\sigma\sigma'(v)}(\vartheta)
							\right\}
						\end{equation}
						
						Let us put this in a form that makes it more explicitly real. We start with
						
						\begin{equation}
							\Sum_{\sigma\in\{0,1\}^N}
							\Sum_{v\in\mathcal{Z}_\sigma}\e^{-\ii\Delta_{\sigma,v}t}f_{\sigma\sigma'(v)}(\vartheta)\underbrace{=}_{\nu=\sigma'(v)}
							\Sum_{\nu\in\{0,1\}^N}	\Sum_{v\in\mathcal{O}_\nu}\e^{\ii\Delta_{\nu,v}t}f_{\nu'(v)\nu}(\vartheta)=
							\Sum_{\nu\in\{0,1\}^N}	\Sum_{v\in\mathcal{O}_\nu}\e^{\ii\Delta_{\nu,v}t}f_{\nu\nu'(v)}(\vartheta).
						\end{equation}
						
						The total occupation becomes
						
						\begin{equation}
							\langle \hat n(t) \rangle = \Sum_{\sigma\in\{0,1\}^N}\left\{
							f_{\sigma\sigma}(\vartheta)+
							2\Sum_{v\in\mathcal{O}_\sigma}\cos\left(\Delta_{\sigma,v}t\right)f_{\sigma\sigma'(v)}(\vartheta)
							\right\}.
						\end{equation}
						
						The first term can be rewritten as
						\begin{equation}
							\Sum_{\sigma\in\{0,1\}^N} 	f_{\sigma\sigma}(\vartheta) = 
								(\Cos)^{2N}\Sum_{p=0}^N\binom{N}{p} (\Tan)^{2p}\left[(N-p)\sin^2\vartheta+p\cos^2\vartheta\right]=
								2N\sin^2\vartheta\cos^2\vartheta
						\end{equation}

						The total occupation becomes
						
\begin{equation}
\label{eq:noftsig}
%n(t) =N\left[1 + (\Sin)^4-\sin^2\vartheta\,\cos^2\vartheta\right]-
\langle \hat n(t) \rangle =2N\sin^2\vartheta\cos^2\vartheta-
2(\Cos)^{2N+2}\Sum_{\sigma\in\{0,1\}^N}(\Tan)^{2n_\sigma}
\Sum_{v\in\mathcal{O}_\sigma}\cos\left(\Delta_{\sigma,v}t\right)
\end{equation}

\paragraph{Remark :} for $n_\sigma = 0$, the term in the sum vanishes $\left(\Sum_{v\in\mathcal{O}_\sigma}\cos\left(\Delta_{\sigma,v}t\right)=0\right)$.

At $t=0$, this becomes
\begin{equation}
n(0) =2N\sin^2\vartheta\cos^2\vartheta-
2(\Cos)^{2N+2}\Sum_{\sigma\in\{0,1\}^N}(\Tan)^{2n_\sigma}n_\sigma
=2N\sin^2\vartheta\cos^2\vartheta-
2(\Cos)^{2}
N\frac{\tan^2\vartheta}{1+\tan^2\vartheta}=0
\end{equation}

\subsubsection{Expression in terms of graph}
	For an induced subgraph $\Graph_\sigma$ of $\Graph$ and a vertex $v\in\vertices_\sigma$, we note $\kappa_\sigma(v)$ the degree of $v$ in $\Graph_\sigma$, and $\kappa(v)$ its degree in $\Graph$. 
	The energy difference between the Ising configurations corresponding to $\Graph_\sigma$ and to $\Graph_\sigma \setminus {v}$ is  $\kappa(v)$.
	The total occupation can then be expressed as 
						
\begin{equation}
\label{eq:noftgraph}
%n_\Graph(t) =N\left(2\sin^4\vartheta+\cos^2\vartheta\right)-
\langle \hat n(t) \rangle_ \Graph =2N\sin^2\vartheta\cos^2\vartheta-
2(\Cos)^{2N+2}\Sum_{\Graph_\sigma\subset\Graph}(\Tan)^{2|\vertices_\sigma|}
\Sum_{v\in\vertices_\sigma}\cos\left(\kappa_{\sigma}(v)t\right).
\end{equation}

We can also express the sum as

\begin{equation}
	\Sum_{\Graph_\sigma\subset\Graph}(\Tan)^{2|\vertices_\sigma|}
\Sum_{v\in\vertices_\sigma}\cos\left(\kappa_{\sigma}(v)t\right) =
\Sum_{v\in\vertices}
\Sum_{\vertices_\sigma\ni v}(\Tan)^{2|\vertices_\sigma|}
\cos\left(\kappa_{\sigma}(v)t\right).
\end{equation}
						
We note $V(v) = \{v'\in\vertices|(v,v')\in\edges\}$ the set of all neighbours of $v$ in $\Graph$, as well as $V_\sigma(v) = \{v'\in\vertices_\sigma|(v,v')\in\edges_\sigma\}$ the set of all neighbours of $v$ in $\Graph_\sigma$, so that\footnote{$|V_\sigma(v)| = \kappa_\sigma(v)$} 
\begin{equation}
\label{eq:cos}
\Sum_{v\in\vertices}
\Sum_{\vertices_\sigma\ni v}(\Tan)^{2|\vertices_\sigma|}
\cos\left(\kappa_{\sigma}(v)t\right)=
\Sum_{v\in\vertices}\Sum_{\omega=0}^{\kappa(v)}
\Sum_{\substack{\vertices_\sigma\ni v|\\\kappa_\sigma(v)=\omega }}(\Tan)^{2|\vertices_\sigma|}
\cos\left(\omega t\right).
\end{equation}

For a given degree $\omega\leq \kappa(v)$, and a given integer $n\geq0$, there are $\binom{N-1-\kappa(v)}{n}\binom{\kappa(v)}{\omega}$ induced subgraphs $\Graph_\sigma$ of size $n+\omega+1$, containing $v$, and in which
$v$ has degree $\omega$. We can then write


\begin{equation}
\Sum_{v\in\vertices}\Sum_{\omega=0}^{\kappa(v)}
\Sum_{\substack{\vertices_\sigma\ni v\\\kappa_\sigma(v)=\omega }}(\Tan)^{2|\vertices_\sigma|}
\cos\left(\omega t\right)=
\Sum_{v\in\vertices}
\underbrace{\Sum_{\omega=0}^{\kappa(v)}\binom{\kappa(v)}{\omega}\cos\left(\omega t\right)(\Tan)^{2\omega+2}}_
	{(\Tan)^2\Re\left\{\left(1+\e^{\ii  t}(\Tan)^2\right)^{\kappa(v)}\right\}}
\underbrace{\Sum_{n=0}^{N-1-\kappa(v)}\binom{N-1-\kappa(v)}{n}(\Tan)^{2n}}_
		{\left(1+(\Tan)^2\right)^{N-1-\kappa(v)}}
\end{equation}

The sum in $\langle \hat n(t) \rangle$ then becomes

\begin{equation}
2(\Cos)^{2N+2}\Sum_{\Graph_\sigma\subset\Graph}(\Tan)^{2|\vertices_\sigma|}
\Sum_{v\in\vertices_\sigma}\cos\left(\kappa_{\sigma}(v)t\right) =
2\,\sin^2\vartheta\Sum_{v\in\vertices}\frac{\Re\left\{\left(1+\e^{\ii  t}\tan^2\vartheta\right)^{\kappa(v)}\right\}}{\left(1+\tan^2\vartheta\right)^{1+\kappa(v)}}.
\end{equation}


If we note $m_\Graph(\kappa)$ the number of vertices of degree $\kappa$ in $\Graph$, and $\kappa_{\max}(\Graph)$ the maximum degree of $\Graph$, 
we can express the occupation as


\begin{equation}
	\label{eq:noft}
\langle \hat n(t) \rangle_ \Graph =
2\,{\sin^2\vartheta\cos^2\vartheta}\Sum_{\kappa=0}^{\kappa_{\max}(\Graph)} m_\Graph(\kappa)\,{\Re\left\{1-\left(\cos^2\vartheta+\e^{\ii  t}\sin^2\vartheta\right)^{\kappa}\right\}}.
\end{equation}


This expression is checked in Fig. \ref{fig:density}, on a random graph of 10 vertices.

\begin{figure}[htpb]
	\centering
	\includegraphics[width=0.6\textwidth]{figures/theory_vs_numerics_density.png}
	\caption{Comparison between \eqref{eq:noft} and numerical simulation of the dynamics, in the case of a density-density hamiltonian, on the graph shown in the inset. Both curves collapse on top
	of each other.}
	\label{fig:density}
\end{figure}


\textbf{Computation for a generic Ising model}
\newline
	We now consider the case of a generic Ising model, defined by the Hamiltonian
	\begin{equation}
		\label{eq:HamIsinggen}
		\Ham_{I_{gen}} = \Sum_{(i,j)\in\edges} J_{ij} \hat n_i \hat n_j + \Sum_{v \in \vertices} h_v \hat n_v.
	\end{equation}
	In this case, \eqref{eq:noftsig} becomes
	\begin{equation}
\langle \hat n(t) \rangle =2N\sin^2\vartheta\cos^2\vartheta-
2(\Cos)^{2N+2}\Sum_{v\in [0,N-1]}\Sum_{\substack{\sigma\in\{0,1\}^N\\ \sigma_v=1}}(\Tan)^{2n_\sigma}\cos\left(\Delta_{\sigma,v}t\right).
	\end{equation}
	We note $\mathcal{N}_\Graph(v) = \left\{v'\in\vertices|(v,v')\in\edges\right\}$ the neighbourhood of $v$ in $\Graph$, and split the Ising configuration $\sigma$ into
	$\sigma = \underbrace{\left\{ \sigma_{v'} | v'\in \mathcal{N}_\Graph(v)\right\}}_{\sigma_{\mathcal{N}_\Graph(v)}}
			\cup \{\sigma_v\}
			\cup
			\underbrace{\left\{ \sigma_{v'} | v'\not\in \mathcal{N}_\Graph(v)\cup\{v\}\right\}}_{\bar\sigma_{\mathcal{N}_\Graph(v)}}$,
	so that
	\begin{equation}
		\Sum_{\substack{\sigma\in\vertices\\ \sigma_v=1}}(\Tan)^{2n_\sigma}\cos\left(\Delta_{\sigma,v}t\right) = 
		\Sum_{\sigma_{\mathcal{N}_\Graph(v)}\in\{0,1\}^{\kappa(v)}}(\Tan)^{2(1+n_{\sigma_{\mathcal{N}_\Graph(v)}})}\cos\left(\Delta_{\sigma,v}t\right)
		\underbrace{\Sum_{\sigma_{\mathcal{N}_\Graph(v)}\in\{0,1\}^{N-1-\kappa(v)}}(\Tan)^{2n_{\bar\sigma_{\mathcal{N}_\Graph(v)}}}}_
		{\left(1+\tan^2\vartheta\right)^{N-\kappa(v)-1}}.
	\end{equation}
	We can then write
	\begin{equation}
		2(\Cos)^{2N+2}\Sum_{v\in \vertices}\Sum_{\substack{\sigma\in\{0,1\}^N\\ \sigma_v=1}}(\Tan)^{2n_\sigma}\cos\left(\Delta_{\sigma,v}t\right)=
		2\cos^2\vartheta\sin^2\vartheta\Sum_{v\in \vertices}\Sum_{\sigma\in\{0,1\}^{\kappa(v)}}\frac{(\Tan)^{2n_{\sigma}}}{\left(1+\tan^2\vartheta\right)^{\kappa(v)}}\cos\left(\Delta_{\sigma,v}t\right).
	\end{equation}
	Finally, we can further simplify the second sum into
	\begin{equation}
		\Sum_{\sigma\in\{0,1\}^{\kappa(v)}}\frac{(\Tan)^{2\Sum_{i=1}^{\kappa(v)} \sigma_{i}}}{\left(1+\tan^2\vartheta\right)^{\kappa(v)}}\cos\left[(h_v+\Sum_{i=1}^{\kappa(v)} J_{v\tilde v_i}\sigma_{i})t\right] =
		\Sum_{\kappa=0}^{\kappa(v)} \frac{(\Tan)^{2\kappa}}{\left(1+\tan^2\vartheta\right)^{\kappa(v)}}\Sum_{\substack{\tilde v\in \mathcal{N}_\Graph(v)^\kappa\\\tilde v_i\neq\tilde v_j}}\cos\left[(h_v+\Sum_{i=1}^\kappa J_{v\tilde v_i})t\right].
	\end{equation}
	Or, 
	\begin{equation}
		\Sum_{\sigma\in\{0,1\}^{\kappa(v)}}\frac{(\Tan)^{2\Sum_{i=1}^{\kappa(v)} \sigma_{i}}}{\left(1+\tan^2\vartheta\right)^{\kappa(v)}}\cos\left[(h_v+\Sum_{i=1}^{\kappa(v)} J_{v\tilde v_i}\sigma_{i})t\right] =
		\Re\left\{\e^{\ii h_v t}
		\Prod_{\tilde v\in\mathcal{N}_\Graph(v)}
		\left(\frac{1+\tan^2\,\vartheta \e^{\ii J_{v\tilde v}t}}{1+\tan^2\vartheta}\right)
		\right\}.
	\end{equation}
	
	The density $\varrho_\Graph(t) = n(t)/N$ then becomes
\begin{equation}
\label{eq:noftgeneric}
\varrho_\Graph(t) =2\sin^2\vartheta\cos^2\vartheta\,\,\Sum_{v\in\vertices}\Re \left\{1-
		\e^{\ii h_v t}\Prod_{\tilde v\in\mathcal{N}_\Graph(v)}
		\left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii J_{v\tilde v}t}}\right)
\right\}
	\end{equation}


	In this form, it is very easy to check that $n(0)=0$.

\textbf{More generic pulse}
\newline We consider here the case where the system is first subject to a $\vartheta$ pulse, then evolves freely for a duration $t$ and finally is subject to a $\varphi$ pulse. In this case the average number of excitations is
\begin{equation}
\langle \hat n(t) \rangle_ \Graph=\sin\vartheta\cos\vartheta\sin\varphi\cos\varphi\,\,\Sum_{v\in\vertices}\Re \left\{\frac{\tan\vartheta}{\tan\varphi}+
        \frac{\tan\varphi}{\tan\vartheta}+
		2\,\,\e^{\ii h_v t}\Prod_{\tilde v\in\vertices}
		\left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii J_{v\tilde v}t}}\right)
\right\}
	\end{equation}

If we consider the case of the uniform local Ising model, \textit{i.e.} $h_v = 1 \forall v \in \mathcal{V}$ and $J_{v_1,v_2}$ is the adjacency matrix of the graph, then we can write :  

\begin{tcolorbox}[ams gather]
\label{eq:noftgeneric}
\langle \hat n(t) \rangle_ \Graph =\sin\vartheta\cos\vartheta\sin\varphi\cos\varphi\,\,\Sum_{v\in\vertices}\Re \left\{\frac{\tan\vartheta}{\tan\varphi}+
        \frac{\tan\varphi}{\tan\vartheta}+
		2\,\,\e^{\ii t} 
		\left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii t}}\right)^{d_v}
\right\}
	\end{tcolorbox}
where $d_v$ is the degree of node $v$. We can see that this quantity is not enough to distinguish two graphs with the same degree histograms, which is the case of two non-isomorphic SRGs from the same family. this completes the first part of the proof.

\subsubsection{Computation of the local observables }
    As we have just shown, the total occupation seems to too simple of an observable to extract meaningful informations from the graph.
    To this end, we express the expectation value of a generic quadratic function of the {\sl bitstring} $\mu$
    \begin{equation}
        \varphi(\mu) = \Sum_{v\in\vertices} h_v \mu_v + \Sum_{(v,v')\in\edges} J_{vv'} \mu_v\mu_{v'}.
    \end{equation}
    
	We start from \eqref{eq:noft_lambda}, and replace $n_\mu$ by $\varphi(\mu)$
	\begin{equation}
	    \label{eq:phiaverage}
	    \begin{aligned}
	    \langle\varphi\rangle(t)=(\Cos)^{2N+3}(\Sin)^3
	                        \Sum_{\mu \in \{0,1\}^N}\varphi(\mu)
	                        \Sum_{\sigma,\sigma'\in\{0,1\}^N} &\e^{-\ii \Delta E_{\sigma\sigma'}t}(\Tan)^{n_\sigma+n_{\sigma'}}\\
							&\times\Prod_{v\in\mathcal{O}_{\sigma\sigma'}}{(\Tan)^{-2{\mu_v}}}
						\Prod_{v\in\mathcal{Z}_{\sigma\sigma'}}{(\Tan)^{2{\mu_v}}}
						\Prod_{v\in\Delta_{\sigma\sigma'}}{(-1)^{{\mu_v}}}.
	    \end{aligned}
	\end{equation}
    
    \textbf{Linear term}
    \newline 
    Let us focus on a given linear term and find an expression for $\langle \mu_v\rangle$. We start from
    \eqref{eq:phiaverage}.

    We note $\mathcal{O}_v=\left\{\sigma\in\{0,1\}^N|\sigma_v=1\right\}$ and $\mathcal{Z}_v=\left\{\sigma\in\{0,1\}^N|\sigma_v=0\right\}$ then expand $\Sum_{\sigma,\sigma'\in\{0,1\}^N}$ into

    
    \textit{The term for $v\in\mathcal{O}_{\sigma\sigma'}$}
    	\begin{equation}
	    \begin{aligned}
			\Sum_{\mu\in\mathcal{O}_{v}} f_{\sigma\sigma'}^\mu(\vartheta)
				&= (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}\Sum_{p_1=0}^{\bf n_1-1} \binom{n_1-1}{p_1}(\Tan)^{-2(p_1+1)}
											\Sum_{p_0=0}^{n_0} \binom{n_0}{p_0}(\Tan)^{2p_0}
											\Sum_{p_{\neq}=0}^{n_{\neq}}(-1)^{p_{\neq}}\\
				&= (\Cos)^{2N}\delta_{\sigma\sigma'}(\Tan)^{2(n_1-1)}(1+\tan^{-2}\vartheta)^{n_1-1}(1+\tan^{2}\vartheta)^{n_0}\\
				&= (\Cos)^{2N}\delta_{\sigma\sigma'}(\Tan)^{2(n_1-1)}(\Sin)^{-2(n_1-1)}(\Cos)^{-2n_0}\\
				&= \delta_{\sigma\sigma'}\cos^2\vartheta
	    \end{aligned}
	\end{equation}
    
    \textit{The term for $v\in\mathcal{Z}_{\sigma\sigma'}$}
    	\begin{equation}
	    \begin{aligned}
			\Sum_{\mu\in\mathcal{O}_{v}} f_{\sigma\sigma'}^\mu(\vartheta)
				&= (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}\Sum_{p_1=0}^{n_1} \binom{n_1}{p_1}(\Tan)^{-2p_1)}
				&= \delta_{\sigma\sigma'}\sin^2\vartheta
	    \end{aligned}
	\end{equation}
	
    \textit{The term for $v\in\Delta_{\sigma\sigma'}$}
    	\begin{equation}
	    \begin{aligned}
			\Sum_{\mu\in\mathcal{O}_{v}} f_{\sigma\sigma'}^\mu(\vartheta)
				&= (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}\Sum_{p_1=0}^{n_1} \binom{n_1}{p_1}(\Tan)^{-2p_1}
											\Sum_{p_0=0}^{n_0} \binom{n_0}{p_0}(\Tan)^{2p_0}
											\Sum_{p_{\neq}=0}^{n_{\neq}-1}(-1)^{p_{\neq}+1}\\
				&= -(\Cos)^{2N}\delta_{n_{\neq}-1}(\Tan)^{1+2n_1}(\Sin)^{-2n_1}(\Cos)^{-2n_0}\\
				&= -\delta_{n_{\neq}-1}\sin\vartheta\cos\vartheta
	    \end{aligned}
	\end{equation}
	
    \textit{The sum of all terms : $  \langle n_{v}(t)\rangle_\Graph$}
    \begin{equation}
	    \begin{aligned}
    		 \langle n_{v}(t)\rangle_\Graph = (\Cos)^{2N}
			&\left[\cos^2\vartheta\Sum_{\sigma\in\mathcal{O}_{v}}\tan^{2n_\sigma}\vartheta
			+\sin^2\vartheta\Sum_{\sigma\in\mathcal{Z}_{v}}{\tan^{2n_\sigma}\vartheta}\right.\\
			&-\sin\vartheta\cos\vartheta\Sum_{\sigma\in\mathcal{O}_{v}}{(\Tan)^{2n_\sigma-1}}\e^{\ii \Delta E_{\sigma\tilde\sigma^v} t}
			-\left.\sin\vartheta\cos\vartheta\e^{\ii h_{v} t}\Sum_{\sigma\in\mathcal{Z}_{v}}{(\Tan)^{2n_\sigma+1}}\e^{-\ii \Delta E_{\sigma\tilde\sigma^v} t}
		\right]
	    \end{aligned}
    \end{equation}
    

    We have introduced here $\tilde\sigma^{v}$ the configuration obtained from $\sigma$ by flipping $\sigma_v$. 

We focus on the first two terms first.

    \begin{equation}
	    \begin{aligned}
			\cos^2\vartheta\Sum_{\sigma\in\mathcal{O}_{v}}\tan^{2n_\sigma}\vartheta
			+\sin^2\vartheta\Sum_{\sigma\in\mathcal{Z}_{v}}\tan^{2n_\sigma}\vartheta
			&=
			\cos^2\vartheta\Sum_{n=0}^{N-1}\binom{N-1}{n}\tan^{2(n+1)}\vartheta
			+\sin^2\vartheta\Sum_{n=0}^{N-1}\binom{N-1}{n}\tan^{2n}\vartheta\\
			&=2\sin^2\vartheta\Sum_{n=0}^{N-1}\binom{N-1}{n}\tan^{2n}\vartheta\\
			&=2\sin^2\vartheta\cos^2\vartheta(\Cos)^{-2N}.
	    \end{aligned}
    \end{equation}
    And now, the third term, using \eqref{eq:HamIsinggen}

    \begin{equation}
	    \begin{aligned}
			\cos^2\vartheta\Sum_{\sigma\in\mathcal{O}_{v}}(\Tan)^{2n_\sigma}\e^{\ii \Delta E_{\sigma\tilde\sigma^v} t}
			&=\sin^2\vartheta\,\e^{\ii h_{v} t}
			\Prod_{\tilde v\in\mathcal{N}_\Graph(v)}\left(1+\tan^2\vartheta\,\e^{\ii J_{\tilde v} t}\right)
			\Sum_{n=0}^{N-1-\kappa(v)}\binom{N-1-\kappa(v)}{n}(\Tan)^{2n}\\
			&=\sin^2\vartheta\,\e^{\ii h_{v} t}
			\Prod_{\tilde v\in\mathcal{N}_\Graph(v)}\left(1+\tan^2\vartheta\,\e^{\ii J_{v\tilde v} t}\right)
			(\Cos)^{2(1+\kappa(v)-N)}\\
			&=\sin^2\vartheta\cos^2\vartheta(\Cos)^{-2N}\,\e^{\ii h_{v} t}
			\Prod_{\tilde v\in\mathcal{N}_\Graph(v)}\left(\cos^2\vartheta+\sin^2\vartheta\,\e^{\ii J_{v\tilde v} t}\right).
	    \end{aligned}
    \end{equation}
    
    Similarly, the fourth terms is

    \begin{equation}
	    \begin{aligned}
			\sin^2\vartheta\Sum_{\sigma\in\mathcal{Z}_{v}}(\Tan)^{2n_\sigma}\e^{-\ii \Delta E_{\sigma\tilde\sigma^v} t}
			&=\sin^2\vartheta\,\e^{-\ii h_{v} t}
			\Prod_{\tilde v\in\mathcal{N}_\Graph(v)}\left(1+\tan^2\vartheta\,\e^{-\ii J_{v\tilde v} t}\right)
			\Sum_{n=0}^{N-1-\kappa(v)}\binom{N-1-\kappa(v)}{n}(\Tan)^{2n}\\
			&=\sin^2\vartheta\,\e^{-\ii h_{v} t}
			\Prod_{\tilde v\in\mathcal{N}_\Graph(v)}\left(1+\tan^2\vartheta\,\e^{-\ii J_{v\tilde v} t}\right)
			(\Cos)^{2(1+\kappa(v)-N)}\\
			&=\sin^2\vartheta\cos^2\vartheta(\Cos)^{-2N}\,\e^{-\ii h_{v} t}
			\Prod_{\tilde v\in\mathcal{N}_\Graph(v)}\left(\cos^2\vartheta+\sin^2\vartheta\,\e^{-\ii J_{v\tilde v} t}\right).
	    \end{aligned}
    \end{equation}

   Adding all those terms together, we get
   
   
\begin{equation}
 \langle n_{v}(t)\rangle_\Graph =2\sin^2\vartheta\cos^2\vartheta\,\,\Re \left\{1-
		\e^{\ii h_v t}\Prod_{\tilde v\in\mathcal{N}_\Graph(v)}
		\left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii J_{v\tilde v}t}}\right)
\right\}
	\end{equation}

\textbf{Quadratic term}
\newline
We no focus on a given quadratic term and find an expression for $\langle \mu_{v_1}\mu_{v_2}\rangle$, where $v_1\neq v_2$. We start from again from 
    \eqref{eq:phiaverage}.
    
    
    \textit{$v_1,v_2\in\mathcal{O}_{\sigma\sigma'}$}
    
    	\begin{equation}
		\begin{aligned}
			\Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta)
				&= (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}\Sum_{p_1=0}^{\bf n_1-2} \binom{n_1-2}{p_1}(\Tan)^{-2(p_1+2)}
											\Sum_{p_0=0}^{n_0} \binom{n_0}{p_0}(\Tan)^{2p_0}
											\Sum_{p_{\neq}=0}^{n_{\neq}}(-1)^{p_{\neq}}\\
				&= \cos^4\vartheta \, \delta_{\sigma\sigma'}
		\end{aligned}
    	\end{equation}
	Note that here $\forall v, \sigma_v=\sigma'_v$, and
	\begin{equation}
		(\Tan)^{n_\sigma+n_{\sigma'}} \Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta) =
			\cos^4\vartheta (\Tan)^{2n_\sigma} \, \delta_{\sigma\sigma'}
	\end{equation}
    
    \textit{$v_1\in\mathcal{O}_{\sigma\sigma'},v_2\in\mathcal{Z}_{\sigma\sigma'}$}
    
    	\begin{equation}
		\begin{aligned}
			\Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta)
				&= (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}\Sum_{p_1=0}^{\bf n_1-1} \binom{n_1-1}{p_1}(\Tan)^{-2(p_1+1)}
											\Sum_{p_0=0}^{\bf n_0-1} \binom{n_0-1}{p_0}(\Tan)^{2(p_0+1)}
											\Sum_{p_{\neq}=0}^{n_{\neq}}(-1)^{p_{\neq}}\\
				&= \sin^2\vartheta\cos^2\vartheta  \,\delta_{\sigma\sigma'}
		\end{aligned}
    	\end{equation}
	Note that here $\forall v, \sigma_v=\sigma'_v$, and
	\begin{equation}
		(\Tan)^{n_\sigma+n_{\sigma'}} \Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta) =
			\cos^4\vartheta (\Tan)^{2n_\sigma+1} \, \delta_{\sigma\sigma'}
	\end{equation}

    \textit{$v_1\in\mathcal{O}_{\sigma\sigma'},v_2\in\Delta_{\sigma\sigma'}$} 
    
    	\begin{equation}
		\begin{aligned}
			\Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta)
				&= (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}\Sum_{p_1=0}^{\bf n_1-1} \binom{n_1-1}{p_1}(\Tan)^{-2(p_1+1)}
											\Sum_{p_0=0}^{n_0} \binom{n_0}{p_0}(\Tan)^{2p_0}
											\Sum_{p_{\neq}=0}^{\bf n_{\neq}-1}(-1)^{p_{\neq}+1}\\
				&=  -\Sin\cos^3\vartheta  \,\delta_{n_{\neq}-1}
		\end{aligned}
    	\end{equation}
	Note that here $\forall v\neq v_2, \sigma_v=\sigma'_v$, and $\sigma_{v_2} = 1-\sigma'_{v_2}$, and
	\begin{equation}
		(\Tan)^{n_\sigma+n_{\sigma'}} \Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta) =
			-\cos^4\vartheta (\Tan)^{2(n_\sigma-\sigma_{v_2})}  \,\delta_{n_{\neq}-1} \, \bar\delta_{\sigma_{v_2}\sigma'_{v_2}}
	\end{equation}
    
    \textit{$v_1,v_2\in\mathcal{Z}_{\sigma\sigma'}$}
    
    	\begin{equation}
		\begin{aligned}
			\Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta)
				&= (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}\Sum_{p_1=0}^{n_1} \binom{n_1}{p_1}(\Tan)^{-2p_1}
											\Sum_{p_0=0}^{\bf n_0-2} \binom{n_0-2}{p_0}(\Tan)^{2(p_0+2)}
											\Sum_{p_{\neq}=0}^{n_{\neq}}(-1)^{p_{\neq}}\\
				&= \sin^4\vartheta  \,\delta_{\sigma\sigma'}
		\end{aligned}
    	\end{equation}
	Note that here $\forall v, \sigma_v=\sigma'_v$, and
	\begin{equation}
		(\Tan)^{n_\sigma+n_{\sigma'}} \Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta) =
			\sin^4\vartheta (\Tan)^{2n_\sigma} \, \delta_{\sigma\sigma'} =
			\cos^4\vartheta (\Tan)^{2n_\sigma+4} \, \delta_{\sigma\sigma'}
	\end{equation}
    
    \textit{$v_1\in\mathcal{Z}_{\sigma\sigma'},v_2\in\Delta_{\sigma\sigma'}$}
    
    	\begin{equation}
		\begin{aligned}
			\Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta)
				&= (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}\Sum_{p_1=0}^{n_1} \binom{n_1}{p_1}(\Tan)^{-2p_1}
											\Sum_{p_0=0}^{\bf n_0-1} \binom{n_0-1}{p_0}(\Tan)^{2(p_0+1)}
											\Sum_{p_{\neq}=0}^{\bf n_{\neq}-1}(-1)^{p_{\neq}+1}\\
				&=  -\sin^3\vartheta\Cos  \,\delta_{n_{\neq}-1}
		\end{aligned}
    	\end{equation}
	Note that here $\forall v\neq v_2, \sigma_v=\sigma'_v$, and $\sigma_{v_2} = 1-\sigma'_{v_2}$, and
	\begin{equation}
		\begin{aligned}
		(\Tan)^{n_\sigma+n_{\sigma'}} \Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta) &=
			-\sin^4\vartheta (\Tan)^{2(n_\sigma-\sigma_{v_2})}  \,\delta_{n_{\neq}-1} \, \bar\delta_{\sigma_{v_2}\sigma'_{v_2}}\\&=
			-\cos^4\vartheta (\Tan)^{2(n_\sigma+2-\sigma_{v_2})}  \,\delta_{n_{\neq}-1} \,\bar \delta_{\sigma_{v_2}\sigma'_{v_2}}
		\end{aligned}
	\end{equation}


    
    \textit{$v_1,v_2\in\Delta_{\sigma\sigma'}$}
    
    	\begin{equation}
		\begin{aligned}
			\Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta)
				&= (\Cos)^{2N}(\Tan)^{n_{\neq}+2n_1}\Sum_{p_1=0}^{n_1} \binom{n_1}{p_1}(\Tan)^{-2p_1}
											\Sum_{p_0=0}^{n_0} \binom{n_0}{p_0}(\Tan)^{2p_0}
											\Sum_{p_{\neq}=0}^{\bf n_{\neq}-2}(-1)^{p_{\neq}+2}\\
				&= \sin^2\vartheta\cos^2\vartheta  \,\delta_{n_{\neq}-2}
		\end{aligned}
    	\end{equation}
	Note that here $\forall v\neq v_2,v_1, \sigma_v=\sigma'_v$, and $\sigma_{v_1} = 1-\sigma'_{v_1}, \sigma_{v_2} = 1-\sigma'_{v_2}$, and
	\begin{equation}
		(\Tan)^{n_\sigma+n_{\sigma'}} \Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta) =
			\cos^4\vartheta (\Tan)^{2(n_\sigma-\sigma_{v_2}-\sigma_{v_2})}  \,\delta_{n_{\neq}-2} \, \bar\delta_{\sigma_{v_2}\sigma'_{v_2}} \,\bar \delta_{\sigma_{v_1}\sigma'_{v_1}}
	\end{equation}
	
    \textit{$ \langle n_{v_1}n_{v_2}(t) \rangle_\Graph$}
    \newline In the following, we will note $\tilde\sigma^i$ the configuration obtained from $\sigma$ by flipping $\sigma_{v_i}$, and $\dbtilde \sigma$ the 
    configuration obtained from $\sigma$ by flipping both $\sigma_{v_1}$ and $\sigma_{v_2}$. We then split the sum $\Sum_{\sigma\in\{0,1\}^N}$ into
    four terms
    \begin{equation}
    \Sum_{\sigma\in \mathcal{O}_{v_1}\cap\mathcal{O}_{v_2} } 
    + \Sum_{\sigma\in \mathcal{O}_{v_1}\cap\mathcal{Z}_{v_2} } 
    + \Sum_{\sigma\in \mathcal{Z}_{v_1}\cap\mathcal{O}_{v_2} }
    +\Sum_{\sigma\in \mathcal{Z}_{v_1}\cap\mathcal{Z}_{v_2} }
    := \mathcal{S}_{11}+\mathcal{S}_{10}+\mathcal{S}_{01}+\mathcal{S}_{00},
    \end{equation}
     and focus on each of them separately.
    
    
    
    \begin{equation}
    	\begin{aligned}
    	\mathcal{S}_{11}&=\Sum_{\sigma\in \mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}}\Sum_{\sigma'\in\{0,1\}^N}
	\e^{-\ii \Delta E_{\sigma,\sigma'} t} (\Tan)^{n_\sigma+n_{\sigma'}} \Sum_{\mu\in\mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}} f_{\sigma\sigma'}^\mu(\vartheta)  \\
				&= \cos^4\vartheta\Sum_{n=0}^{N-2} \binom{N-2}{n}(\Tan)^{2(n+2)}\\
				&- \cos^4\vartheta\Sum_{\sigma\in \mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}}(\Tan)^{2(n_\sigma-1)}
						\left(\e^{-\ii \Delta E_{\sigma,\tilde\sigma^1} t}+\e^{-\ii \Delta E_{\sigma,\tilde\sigma^2} t}\right)\\
				&+\cos^4\vartheta \Sum_{\sigma\in \mathcal{O}_{v_1}\cap\mathcal{O}_{v_2}}(\Tan)^{2n_\sigma}\e^{-\ii \Delta E_{\sigma,\dbtilde\sigma} t}
    	\end{aligned}
    \end{equation}
				
				
    
    We introduce $\mathcal{N}_{12}=\mathcal{N}_\Graph(v_1)\cap\mathcal{N}_\Graph(v_2)$, and 
    $\mathcal{N}_{1}=\mathcal{N}_\Graph(v_1)\backslash\mathcal{N}_{12}\backslash v_2$ (and $1\leftrightarrow2$).
    Furthermore, we also introduce 
    \begin{equation}
    	w_\vartheta( \phi, t ) = \left(\cos^2\vartheta + \sin^2\vartheta \, \e^{-\ii \phi t}\right)
    \end{equation}
    
      If $(v_1,v_2)\in\edges$, then
    \begin{equation}
    	\begin{aligned}
    	\mathcal{S}_{11}&=(\Cos)^{-2N}\sin^2\vartheta\cos^6\vartheta\left[\tan^2\vartheta
					-\e^{-\ii h_{v_1} t}\Prod_{\tilde v \in \mathcal{N}\backslash v_2}w_\vartheta( J_{v_1\tilde v}, t )%\left(\cos^2\vartheta + \sin^2\vartheta \, \e^{-\ii J_{v_1\tilde v} t}\right)
%				&
					-\e^{-\ii h_{v_2} t}\Prod_{\tilde v \in \mathcal{N}\backslash v_1}w_\vartheta( J_{v_2\tilde v}, t )%\left(\cos^2\vartheta + \sin^2\vartheta \, \e^{-\ii J_{v_2\tilde v} t}\right)
					\right.\\
					&
					\left.
					+\tan^2\vartheta \,\e^{-\ii (h_{v_1}+h_{v_2} + J_{v_1v_2}) t}
					\Prod_{\tilde v \in \mathcal{N}_1}w_\vartheta( J_{v_1\tilde v}, t )%  \left(\cos^2\vartheta + \sin^2\vartheta \, \e^{-\ii J_{v_1\tilde v} t}\right)
					\Prod_{\tilde v \in \mathcal{N}_2}w_\vartheta( J_{v_2\tilde v}, t )%\left(\cos^2\vartheta + \sin^2\vartheta \, \e^{-\ii J_{v_2\tilde v} t}\right)
					\Prod_{\tilde v \in \mathcal{N}_{12}}w_\vartheta( J_{v_1\tilde v} + J_{v_2\tilde v}, t )%\left(\cos^2\vartheta + \sin^2\vartheta \, \e^{-\ii (J_{v_1\tilde v}+J_{v_2\tilde v}) t}\right)
				\right]
    	\end{aligned}
    \end{equation}    

				
	The generic expression is
    \begin{equation}
    	\begin{aligned}
    	\mathcal{S}_{11}&=(\Cos)^{-2N}\sin^2\vartheta\cos^6\vartheta\left[\tan^2\vartheta
					-\e^{-\ii h_{v_1} t}\Prod_{\tilde v \neq v_2}w_\vartheta( J_{v_1\tilde v}, t )
					-\e^{-\ii h_{v_2} t}\Prod_{\tilde v \neq v_1}w_\vartheta( J_{v_2\tilde v}, t )
					\right.\\
					&
					\left.
					+\tan^2\vartheta \,\e^{-\ii (h_{v_1}+h_{v_2} + J_{v_1v_2}) t}
					\Prod_{\tilde v \neq v_1,v_2}w_\vartheta( J_{v_1\tilde v} + J_{v_2\tilde v}, t )
					\right]
    	\end{aligned}
    \end{equation}    
    
    	
    \begin{equation}
    	\begin{aligned}
    	\mathcal{S}_{10}&=(\Cos)^{-2N}\sin^2\vartheta\cos^6\vartheta\left[\tan\vartheta
					-\e^{\ii h_{v_2} t}\Prod_{\tilde v \neq v_1}w_\vartheta( -J_{v_2\tilde v}, t )\right.\\
					&-\tan^{-1}\vartheta\e^{-\ii h_{v_1} t}\Prod_{\tilde v \neq v_2}w_\vartheta( J_{v_1\tilde v}, t )\\
					&-\tan^{-2}\vartheta\e^{-\ii h_{v_1} t}\Prod_{\tilde v \neq v_2}w_\vartheta( J_{v_1\tilde v}, t )\\
					&
					\left.
					+\tan^2\vartheta \,\e^{-\ii (h_{v_1}+h_{v_2} + J_{v_1v_2}) t}
					\Prod_{\tilde v \neq v_1,v_2}w_\vartheta( J_{v_1\tilde v} + J_{v_2\tilde v}, t )
					\right]
    	\end{aligned}
    \end{equation}    
    

    
    
   
   
\begin{equation}
		\begin{aligned}
\langle n_{v_1}n_{v_2}(t)\rangle_\Graph =4\sin^4\vartheta\cos^4\vartheta\,\,\Re &\left\{1
		-\e^{\ii h_{v_1} t}\Prod_{\tilde v\neq v_2}\left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii J_{v_1\tilde v}t}}\right)
		-\e^{\ii h_{v_2} t}\Prod_{\tilde v\neq v_1}\left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii J_{v_2\tilde v}t}}\right)\right.\\
		&+\frac{1}{2}\e^{\ii (h_{v_1}+h_{v_2} +J_{v_1v_2}) t}\Prod_{\tilde v\neq v_1,v_2}\left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii (J_{v_1\tilde v}+J_{v_2\tilde v})t}}\right)\\
		&\left.+\frac{1}{2}\e^{\ii (h_{v_1}-h_{v_2}) t}\Prod_{\tilde v\neq v_1,v_2}\left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii (J_{v_1\tilde v}-J_{v_2\tilde v})t}}\right)
\right\}
		\end{aligned}
	\end{equation}

  
  \textit{$\langle n_{v_1}n_{v_2}(t)\rangle_\Graph - \langle n_{v_1}(t)\rangle_\Graph\langle n_{v_2}(t)\rangle_\Graph$}
  
  In order to emphasise the structure of the expression, we introduce
  
  \begin{equation}
  	w_{v\tilde v}(\vartheta,t) = \left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii J_{v\tilde v}t}}\right)
  \end{equation}
  
  and 
  
  \begin{equation}
  	\varrho_{\vartheta,v}(t) = \e^{\ii h_{v_1} t}\Prod_{\tilde v}\left({\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii J_{v\tilde v}t}}\right) = \e^{\ii h_{v_1} t}\Prod_{\tilde v} w_{v\tilde v}(\vartheta,t),
  \end{equation}
  
  so that
  
  \begin{equation}
\langle n_{v}(t)\rangle_\Graph =2\sin^2\vartheta\cos^2\vartheta\,\,\Re \left\{1-\varrho_{\vartheta,v}(t)\right\} = 2\sin^2\vartheta\cos^2\vartheta\left[1-\frac{1}{2}\left(\varrho_{\vartheta,v}(t)+\varrho^*_{\vartheta,v}(t)\right)\right],
\end{equation}

and 
  
  \begin{equation}
\langle n_{v_1}n_{v_2}(t)\rangle_\Graph =4\sin^4\vartheta\cos^4\vartheta\,\,\Re \left\{1
												-\left[\varrho_{\vartheta,v_1}(t)+\varrho_{\vartheta,v_2}(t)\right]
												+\frac{1}{2}\left[\varrho_{\vartheta,v_1}(t)\varrho_{\vartheta,v_2}(t)+\varrho_{\vartheta,v_1}(t)\varrho^*_{\vartheta,v_2}(t)\right]\right\}.
\end{equation}




Similarly,
  \begin{equation}
  \begin{aligned}
\langle n_{v_1}n_{v_2}(t)\rangle_\Graph =4\sin^4\vartheta\cos^4\vartheta\,\,\Re 
		&\left\{1-\frac{\varrho_{\vartheta,v_1}(t)+\varrho_{\vartheta,v_2}(t)}{w_{v_1v_2}(\vartheta,t)}\right.\\
		&+\frac{1}{2}\e^{\ii J_{v_1v_2}t}\frac{\varrho_{\vartheta,v_1}(t)\varrho_{\vartheta,v_2}(t)}
				{\Prod_{\tilde v \in \mathcal{N}_{12}\cup \{v_1,v_2\}}  \cos^2\vartheta+\sin^2\vartheta\;\e^{\ii (J_{v_1\tilde v}+J_{v_2\tilde v})t}}\\
		&\left.+\frac{1}{2}\frac{\varrho_{\vartheta,v_1}(t)\varrho_{\vartheta,v_2}^*(t)}
				{\Prod_{\tilde v \in \mathcal{N}_{12}\cup \{v_1,v_2\}}  \cos^2\vartheta+\sin^2\vartheta\;\e^{\ii (J_{v_1\tilde v}-J_{v_2\tilde v})t}}
\right\}.
\end{aligned}
\end{equation}

Introducing $w^{\pm}_{v1v_2}(\vartheta,t)=\Prod_{\tilde v \in \mathcal{N}_{12}\cup \{v_1,v_2\}}\cos^2\vartheta+\sin^2\vartheta\;\e^{\ii (J_{v_1\tilde v}\pm J_{v_2\tilde v})t}$, the correlation between densities at $v_1$ and $v_2$ can then be expressed as

\begin{tcolorbox}
\begin{align}
\langle n_{v_1}n_{v_2}(t)\rangle_\Graph -\langle n_{v_1}(t)\rangle_\Graph\langle n_{v_2}(t)\rangle_\Graph=4\sin^4\vartheta\cos^4\vartheta\,\,\Re 
		&\left\{\left[\varrho_{\vartheta,v_1}(t)+\varrho_{\vartheta,v_2}(t)\right]\left[1-w_{v_1v_2}(\vartheta,t)^{-1}\right]\right. \nonumber \\
		&+\frac{1}{2}\left[1-\e^{\ii J_{v_1v_2}t} w^+_{v_1v_2}(\vartheta,t)^{-1}\right]
		\varrho_{\vartheta,v_1}(t)\varrho_{\vartheta,v_2}(t) \nonumber \\
		&\left.+\frac{1}{2}\left[1- w^-_{v_1v_2}(\vartheta,t)^{-1}\right]
		    \varrho_{\vartheta,v_1}(t)\varrho_{\vartheta,v_2}^*(t)
\right\}.
\label{eq:generic_corr}
\end{align}
\end{tcolorbox}

Since we consider only the uniform Ising model for this proof, we have $h_v = 1 \; \forall v \in \mathcal{V}$ and $J_{v_1,v_2} = 1 $ if $(v_1,v_2) \in \mathcal{E}$ and $0$ if not. This allows us to rewrite the elements recovered in the generic expression derived in equation \ref{eq:generic_corr} as : 

\begin{itemize} 
\item $\varrho_{\vartheta,v}(t) = (\cos^2\vartheta + \sin^2\vartheta e^{\ii t})^{d_v}$
\item $w^{+}_{v1,v_2}(\vartheta,t) = (\cos^2\vartheta + \sin^2\vartheta e^{2\ii t})^{\Gamma_{v_1,v_2}}.(\cos^2\vartheta + \sin^2\vartheta e^{\ii t})^{2.J_{v_1,v_2}}$
\item $ w^{-}_{v1,v_2}(\vartheta,t) = (\cos^2\vartheta + \sin^2\vartheta e^{2\ii t})^{\Gamma_{v_1,v_2}}.\left[(\cos^2\vartheta + \sin^2\vartheta e^{-\ii t}) .(\cos^2\vartheta + \sin^2\vartheta e^{\ii t}) \right]^{J_{v_1,v_2}} $
\end{itemize}

These elements are explicitly dependent of the elements of the adjacency matrix $J_{v_1,v_2}$ of the graph, as well as the degree of each node $d_v$, and the number $\Gamma_{v_1,v_2}$ of common neighbors between nodes $v_1$ and $v_2$. Thus we cans easily verify that the correlation matrix is going to be the same for two non-isomorphic SRGs, as it only depends on two of the invariants of the family, namely the degree and number of comon neighbors, as defined in \ref{{def:SRGs}}. This completes the proof for the proposition \ref{pr:GD-Ising}. 






    
\end{document}


